Multiple Subspace Alignment Improves Domain Adaptation

We present a novel unsupervised domain adaptation (DA) method for cross-domain visual recognition. Though subspace methods have found success in DA, their performance is often limited due to the assumption of approximating an entire dataset using a single low-dimensional subspace. Instead, we develop a method to effectively represent the source and target datasets via a collection of low-dimensional subspaces, and subsequently align them by exploiting the natural geometry of the space of subspaces, on the Grassmann manifold. We demonstrate the effectiveness of this approach, using empirical studies on two widely used benchmarks, with state of the art domain adaptation performance

==> related_work.tex <==
There are fundamentally two main aspects that need to be addressed in order to solve domain adaptation -- (a) representation of the datasets, and (b) alignment of the source and target distributions, and most existing techniques essentially vary in their choice of representation and alignment.  Subspace based methods represent the datasets using a single subspace  \cite{Fernando2014SubspaceAF,DBLP:conf/iccv/FernandoHST13, Gong2012GeodesicFK, ShrivastavaWACV2014}, while solving different kinds of alignment between the source and target subspaces. However, restricting to just a single subspace severely restricts the representation capacity of such subspace based methods. More recently, optimal transport has proven to be a powerful alignment strategy regardless of how the datasets are represented \cite{seguy2017large,,}. Further, domain adaptation using adversarial training, has proven to be a powerful way to jointly solve the representation and alignment steps \cite{tzeng2017adversarial,,}, but these methods require large datasets and need the source and target to be jointly trained, which maybe unrealistic in several scenarios.

